Gradient-based dimension reduction of multivariate vector-valued functions

Multivariate functions encountered in high-dimensional uncertainty quantification problems often vary most strongly along a few dominant directions in the input parameter space. We propose a gradient-based method for detecting these directions and using them to construct ridge approximations of such functions, in the case where the functions are vector-valued (e.g., taking values in $\mathbb{R}^n$). The methodology consists of minimizing an upper bound on the approximation error, obtained by subspace Poincar\'e inequalities. We provide a thorough mathematical analysis in the case where the parameter space is equipped with a Gaussian probability measure. The resulting method generalizes the notion of active subspaces associated with scalar-valued functions. A numerical illustration shows that using gradients of the function yields effective dimension reduction. We also show how the choice of norm on the codomain of the function has an impact on the function's low-dimensional approximation.

==> 19-10-08 Final version/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
% \usepackage{lipsum}
\usepackage[utf8]{inputenc} % for french accents

% \usepackage[centering]{geometry}
% \geometry{textheight=8in,textwidth=5.5in}

% \setlength{\marginparwidth}{2.5cm}

% \usepackage[textsize=tiny,textwidth=2cm]{todonotes}
\usepackage{mathtools}
\usepackage{color}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{tikz,pgfplots}
\newlength\figheight
\newlength\figwidth

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Gradient-based dimension reduction}{O.~Zahm, P.~Constantine, C.~Prieur, Y.~Marzouk}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Gradient-based dimension reduction of multivariate vector-valued functions
\thanks{Submitted to the editors on 20 October  2018.
% \funding{This work was funded by......}
}}

% Authors: full names plus addresses.
\author{
  Olivier Zahm\thanks{Univ. Grenoble Alpes, Inria, CNRS, Grenoble INP (Institute of Engineering Univ. Grenoble Alpes), LJK, 38000 Grenoble, France \email{olivier.zahm@inria.fr}}
  \and
  Paul Constantine\thanks{University of Colorado Boulder, \email{paul.constantine@colorado.edu}}
  \and
  Cl\'ementine Prieur\thanks{Univ. Grenoble Alpes, CNRS, Inria, Grenoble INP (Institute of Engineering Univ. Grenoble Alpes), LJK, Grenoble 38000, France \email{clementine.prieur@univ-grenoble-alpes.fr}}
  \and
  Youssef Marzouk\thanks{Massachusetts Institute of Technology, \email{ymarz@mit.edu}}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\Var}{Var}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}

%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> 19-10-08 Final version/graphs/tikz2pdf/UB_H1/UB_H1.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.50000,0.37241}%
\definecolor{mycolor2}{rgb}{1.00000,0.10345,0.72414}%
\definecolor{mycolor3}{rgb}{1.00000,0.82759,0.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
xmin=0,
xmax=300,
xlabel={rank $r$ of the projector},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
% ylabel={upper bound},
axis background/.style={fill=white},
legend style={at={(0.03,0.03)},anchor=south west,legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=blue,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.842657915792269\\
5	0.69076411328902\\
10	0.567914384342777\\
15	0.476785924557505\\
20	0.406368006623714\\
25	0.347900785572591\\
30	0.301806303577856\\
35	0.262880488099575\\
40	0.230194014045033\\
45	0.202513741162513\\
50	0.178147717427282\\
55	0.156988342568957\\
60	0.138168781608234\\
65	0.12109181853017\\
70	0.106528926425554\\
75	0.0936889419612097\\
80	0.0822665056715205\\
85	0.0720300412809685\\
90	0.0633792683428896\\
95	0.0556873697940693\\
100	0.0485950023901831\\
105	0.0425971191201518\\
110	0.0375603788270293\\
115	0.032882828670963\\
120	0.0288230523719433\\
125	0.0252807518472025\\
130	0.0222848255191372\\
135	0.0195927755434287\\
140	0.0171930027056383\\
145	0.0150596473004764\\
150	0.0133468049840736\\
155	0.0117440098319116\\
160	0.0102925419682097\\
165	0.00903941276797616\\
170	0.0079972170917804\\
175	0.00705828060525645\\
180	0.0062173490309346\\
185	0.00546201166393073\\
190	0.00481435025622517\\
195	0.00425947959862928\\
200	0.00377806913410259\\
205	0.00332623911584736\\
210	0.00291985567274236\\
215	0.00257926568453537\\
220	0.00229218502648345\\
225	0.0020334824664312\\
230	0.00178818117580089\\
235	0.00157822061963942\\
240	0.0013953296768144\\
245	0.00123593761551859\\
250	0.00109996239613032\\
255	0.000972228122646838\\
260	0.000861333853902723\\
265	0.000759495833718544\\
270	0.000670261084633744\\
275	0.000598986120236976\\
280	0.000533115877666115\\
285	0.00047226132625629\\
290	0.000417678169458706\\
295	0.000368127814979725\\
300	0.000327672127950067\\
};
\addplot [color=blue,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.858233313722005\\
5	0.726710500676723\\
10	0.611331861835439\\
15	0.521440641551332\\
20	0.45073280005378\\
25	0.39162090729242\\
30	0.345153103193509\\
35	0.304971882449891\\
40	0.272201950431809\\
45	0.241931592771057\\
50	0.214671750368154\\
55	0.189403386423354\\
60	0.166342834561152\\
65	0.145484504191848\\
70	0.12785939489447\\
75	0.112970220789883\\
80	0.0978550357623193\\
85	0.0844639651063895\\
90	0.0741034927655092\\
95	0.0650777186878532\\
100	0.0565137933249781\\
105	0.0493996600070602\\
110	0.0436946809081395\\
115	0.0383440374648774\\
120	0.0335924620857466\\
125	0.0293265542662369\\
130	0.0259297270809694\\
135	0.0228495885241513\\
140	0.0200756147120758\\
145	0.0175363988923956\\
150	0.0155783076410874\\
155	0.0137173356801225\\
160	0.0119984449607093\\
165	0.0105420182906345\\
170	0.00933558145968237\\
175	0.00825588050195221\\
180	0.00727847411198366\\
185	0.00638489820907557\\
190	0.00563014126307845\\
195	0.00498405141256306\\
200	0.0044220138444447\\
205	0.003885310132755\\
210	0.00341673926740516\\
215	0.00302753501577763\\
220	0.00267909295708271\\
225	0.00238438762263271\\
230	0.00209486167654273\\
235	0.00185560976402689\\
240	0.00163960564885917\\
245	0.00144483951843683\\
250	0.00129168246407706\\
255	0.00114373890309044\\
260	0.00101126630068726\\
265	0.000892086551254905\\
270	0.000786292266029136\\
275	0.000704618029058656\\
280	0.000627226236147052\\
285	0.000555613875120688\\
290	0.000492746802403779\\
295	0.000434113607784357\\
300	0.000384968262383339\\
};
\addlegendentry{$K=5$};

\addplot [color=red,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.850512170978715\\
5	0.704704822813094\\
10	0.587794749289308\\
15	0.49533856183076\\
20	0.425080438191743\\
25	0.367428614993631\\
30	0.321040212251133\\
35	0.281075088566629\\
40	0.24684652965523\\
45	0.216763713443671\\
50	0.190413969097751\\
55	0.167226072559285\\
60	0.146722954921339\\
65	0.128456906202566\\
70	0.113053658425114\\
75	0.0996568602030031\\
80	0.0877291179281566\\
85	0.0766816025439446\\
90	0.0677003852937802\\
95	0.0596256659091653\\
100	0.0521824430581325\\
105	0.0457688589507645\\
110	0.0403541725575453\\
115	0.0354679665731202\\
120	0.0311037695542205\\
125	0.027215061905272\\
130	0.0240867563111981\\
135	0.0211795488558973\\
140	0.018541865662408\\
145	0.0162898122777316\\
150	0.0144080240555982\\
155	0.0126994749885521\\
160	0.0111586684930419\\
165	0.00979112418483664\\
170	0.00864364937975739\\
175	0.00765472694217975\\
180	0.00674730400455183\\
185	0.00593119823132425\\
190	0.00522002436231317\\
195	0.00461391729949155\\
200	0.00410160400566164\\
205	0.00361555638665624\\
210	0.00317669498007517\\
215	0.00280674084918528\\
220	0.00248359065132361\\
225	0.00221021578136214\\
230	0.0019487177815258\\
235	0.00171980085126473\\
240	0.00151640268202168\\
245	0.00134092390779691\\
250	0.00119793275704856\\
255	0.00106072078559652\\
260	0.000937748840516486\\
265	0.000827887326621959\\
270	0.000730628168773174\\
275	0.000651960850147478\\
280	0.000579634324411948\\
285	0.000514703528525368\\
290	0.000456163726664842\\
295	0.000402546054791443\\
300	0.000356461480351224\\
};
\addplot [color=red,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.855343515422925\\
5	0.724869593429108\\
10	0.612727575236856\\
15	0.520714012013864\\
20	0.452827595542844\\
25	0.393875659404952\\
30	0.347562169266582\\
35	0.30493893684953\\
40	0.270475138419713\\
45	0.237625916154073\\
50	0.210881081294697\\
55	0.184505415143302\\
60	0.162734053981169\\
65	0.143153568131332\\
70	0.126287500652215\\
75	0.110828825626618\\
80	0.0961926060829579\\
85	0.0837952022864943\\
90	0.0731685820971639\\
95	0.0643951565381324\\
100	0.0555736939276209\\
105	0.0486714637201366\\
110	0.0430127235608683\\
115	0.037580467399705\\
120	0.0329725867095308\\
125	0.0288496066814833\\
130	0.0256019535187486\\
135	0.0224290629797684\\
140	0.0197194190411469\\
145	0.0172799362673527\\
150	0.0153142443176654\\
155	0.0134745158263707\\
160	0.011814359465228\\
165	0.0103577623227093\\
170	0.00917769743068845\\
175	0.00809918537100417\\
180	0.0071530267468867\\
185	0.00627867478167502\\
190	0.00553283416842909\\
195	0.00488868835961701\\
200	0.00434880196089137\\
205	0.00381400169911119\\
210	0.0033564690443103\\
215	0.0029733832890057\\
220	0.0026274429146738\\
225	0.00234488091893221\\
230	0.00205828120847078\\
235	0.00181791315163297\\
240	0.00160556627062258\\
245	0.00142044980028128\\
250	0.00126984671421342\\
255	0.00112296188896457\\
260	0.000993302940352323\\
265	0.000875923354297582\\
270	0.000772835927783662\\
275	0.000690952694755479\\
280	0.000613931429928853\\
285	0.000544293067220917\\
290	0.000483015988450625\\
295	0.000426092175290265\\
300	0.000377510484782385\\
};
\addlegendentry{$K=10$};

\addplot [color=green,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.854197254907859\\
5	0.717015641320805\\
10	0.59634035068928\\
15	0.499413294138865\\
20	0.428333424520721\\
25	0.368839914040255\\
30	0.322536330839426\\
35	0.282091417730032\\
40	0.248324404494851\\
45	0.218369444101101\\
50	0.192034499612396\\
55	0.168156504880067\\
60	0.148037242228472\\
65	0.129462941372921\\
70	0.113726764304868\\
75	0.100006740570129\\
80	0.0876291445270227\\
85	0.0765842557687437\\
90	0.0673473721892849\\
95	0.0593034310290491\\
100	0.0516967704807667\\
105	0.0453185105351316\\
110	0.0400448307415058\\
115	0.0350192675684505\\
120	0.0307308448208458\\
125	0.0269164001636126\\
130	0.0237718111375801\\
135	0.0209047761567915\\
140	0.0183482271438447\\
145	0.0160932478320694\\
150	0.0142603228587902\\
155	0.0125462261165772\\
160	0.0109947189496498\\
165	0.00966226175691337\\
170	0.00854428421407931\\
175	0.00754614105559317\\
180	0.00665564156517151\\
185	0.00584764429501224\\
190	0.00515199682148927\\
195	0.00455976761707171\\
200	0.00404681372373042\\
205	0.00355901960551115\\
210	0.00312853188747008\\
215	0.00276720023033176\\
220	0.00244967361798865\\
225	0.00217965824027847\\
230	0.00191559258221392\\
235	0.00169307677352023\\
240	0.00149492354418456\\
245	0.00132340605749643\\
250	0.00117941719108671\\
255	0.00104521160923427\\
260	0.000923088794761547\\
265	0.000814938953051759\\
270	0.000719386959364935\\
275	0.00064309926084529\\
280	0.000570990551559929\\
285	0.000506878846877783\\
290	0.000449045741468337\\
295	0.000396349116198688\\
300	0.000351318234312536\\
};
\addplot [color=green,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.854271536293235\\
5	0.720938822257353\\
10	0.603114708679451\\
15	0.511065854152822\\
20	0.440297997506645\\
25	0.381167287913049\\
30	0.334852375628686\\
35	0.293337949022501\\
40	0.258378170647058\\
45	0.22683589438385\\
50	0.199507249854882\\
55	0.174596372398823\\
60	0.153595451700334\\
65	0.134275202894173\\
70	0.117690279893938\\
75	0.103466873953241\\
80	0.0904746480054325\\
85	0.0790348430749354\\
90	0.0694357121828301\\
95	0.0611490402694152\\
100	0.0532421550548823\\
105	0.0467003479778135\\
110	0.0413131134014289\\
115	0.0361059575561718\\
120	0.0317100760554909\\
125	0.0277403064309615\\
130	0.0245233024654611\\
135	0.021572687038846\\
140	0.0189333225734948\\
145	0.01660108943279\\
150	0.0147116010715365\\
155	0.012936638101999\\
160	0.011347406156045\\
165	0.00996386032057872\\
170	0.00881598219158893\\
175	0.0077871527292144\\
180	0.00687475828302562\\
185	0.00603073554702547\\
190	0.00531881587345212\\
195	0.00470683406858858\\
200	0.00417673395611798\\
205	0.00367128860650577\\
210	0.00323082673664848\\
215	0.0028601382384628\\
220	0.00252856351067335\\
225	0.002250481372068\\
230	0.00197872797106933\\
235	0.00174817575966883\\
240	0.00154384870534236\\
245	0.00136626119304521\\
250	0.00121864679197393\\
255	0.00107943756435262\\
260	0.000953263631194261\\
265	0.000841566696402781\\
270	0.000743011725841534\\
275	0.000664354421336633\\
280	0.000589681229598217\\
285	0.000523486320278789\\
290	0.000464155885235831\\
295	0.000409346047839079\\
300	0.000362893456377389\\
};
\addlegendentry{$K=30$};

\addplot [color=mycolor1,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.854386196670471\\
5	0.715829649100455\\
10	0.596337164657909\\
15	0.505257296674348\\
20	0.434551537931627\\
25	0.375840497912689\\
30	0.329091227885687\\
35	0.287796761546291\\
40	0.253487154858986\\
45	0.222831622487031\\
50	0.19593373286107\\
55	0.171856239326413\\
60	0.151301077799753\\
65	0.132345716144113\\
70	0.116050989846006\\
75	0.101997903241386\\
80	0.0893180134554772\\
85	0.0780681361709636\\
90	0.0685953782731605\\
95	0.0603877384398105\\
100	0.052672577820526\\
105	0.046161729499692\\
110	0.0408323272764152\\
115	0.0357300118287717\\
120	0.0313569850168351\\
125	0.0274416367499373\\
130	0.0242522639049808\\
135	0.0213346361314315\\
140	0.0187225610812257\\
145	0.0164133581161134\\
150	0.0145474214816311\\
155	0.01279441495011\\
160	0.0112216350886429\\
165	0.0098576077552613\\
170	0.00871647853622832\\
175	0.0077007169598588\\
180	0.00679606340443839\\
185	0.00596871467957036\\
190	0.00525736485084279\\
195	0.00465118921648993\\
200	0.00412990929599793\\
205	0.00363186289061616\\
210	0.00319393569100844\\
215	0.00282538487588462\\
220	0.00249968941170571\\
225	0.00222490526771252\\
230	0.00195610944278869\\
235	0.0017284179297172\\
240	0.00152598562470489\\
245	0.00135011845307759\\
250	0.00120416834912026\\
255	0.00106666276507667\\
260	0.000942489957259844\\
265	0.000831974240424698\\
270	0.000734432222869185\\
275	0.000656132863661093\\
280	0.000582842687974233\\
285	0.000517338293399388\\
290	0.000458485540542471\\
295	0.000404681489306519\\
300	0.000358525052979575\\
};
\addplot [color=mycolor1,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.853612718684342\\
5	0.716122542775951\\
10	0.598343490726109\\
15	0.508100273854599\\
20	0.437429247185325\\
25	0.37831299337161\\
30	0.331995639706559\\
35	0.290444719574667\\
40	0.2558102468566\\
45	0.224630544411742\\
50	0.197707075621589\\
55	0.173045583837339\\
60	0.152329444559517\\
65	0.133120852214766\\
70	0.116674629645553\\
75	0.102613486486817\\
80	0.0897623029108835\\
85	0.0784644201747734\\
90	0.0689223517786045\\
95	0.0606960007209518\\
100	0.0528856073931253\\
105	0.0463870020985316\\
110	0.0410315119051452\\
115	0.0358655495010453\\
120	0.0314980584533803\\
125	0.0275468955104903\\
130	0.0243485092274989\\
135	0.0214278854158599\\
140	0.018796810386387\\
145	0.0164774154883472\\
150	0.0146033015674753\\
155	0.0128439669622764\\
160	0.0112651898774632\\
165	0.00989038705871587\\
170	0.00874914359348096\\
175	0.00773155219608285\\
180	0.00682376333010509\\
185	0.00598693047467329\\
190	0.00527766953456218\\
195	0.00467177462688175\\
200	0.0041437950750276\\
205	0.00364445619186028\\
210	0.00320665092965731\\
215	0.00283843431808208\\
220	0.00250948313530694\\
225	0.002233491085547\\
230	0.00196402968397093\\
235	0.00173481246953296\\
240	0.00153159338331823\\
245	0.00135573646169466\\
250	0.00120928658783182\\
255	0.00107080798966196\\
260	0.000945943900016803\\
265	0.000835083336648327\\
270	0.000737240704930835\\
275	0.000658961819804986\\
280	0.000585130204741495\\
285	0.00051943765284706\\
290	0.000460388465159522\\
295	0.000406074898741922\\
300	0.000360054511064979\\
};
\addlegendentry{$K=100$};

\addplot [color=mycolor2,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.854439098991967\\
5	0.717314039650185\\
10	0.598999906232932\\
15	0.507625162631154\\
20	0.437175784457431\\
25	0.377904176170278\\
30	0.331311201205422\\
35	0.289702904573772\\
40	0.254872064554143\\
45	0.223864678259842\\
50	0.196988836467743\\
55	0.172622774019459\\
60	0.151929224683754\\
65	0.132865093949645\\
70	0.116447433279757\\
75	0.10240101224587\\
80	0.0895604541466094\\
85	0.0782618616135494\\
90	0.0687776858075612\\
95	0.0605399467241175\\
100	0.0528011075011571\\
105	0.0462856095603078\\
110	0.0409424038120007\\
115	0.0358083132010283\\
120	0.0314381319041955\\
125	0.027509517282882\\
130	0.0243103362246009\\
135	0.0213852088507478\\
140	0.018766798421279\\
145	0.0164536087038316\\
150	0.0145890214124435\\
155	0.0128245668503279\\
160	0.0112457331747136\\
165	0.00987848361364716\\
170	0.00873970525857594\\
175	0.00771810401514336\\
180	0.00681152970316948\\
185	0.00598098247437613\\
190	0.00526993326255038\\
195	0.00466607400740655\\
200	0.00413798758146018\\
205	0.00364002499811922\\
210	0.00320119482997444\\
215	0.0028345259470569\\
220	0.0025065699033971\\
225	0.00223012883874875\\
230	0.00196059980242888\\
235	0.00173235763439631\\
240	0.00152952119928271\\
245	0.00135371910019878\\
250	0.00120746291525698\\
255	0.00106932620178584\\
260	0.000944559887812081\\
265	0.000833837423747803\\
270	0.000736177656942217\\
275	0.000657895529395546\\
280	0.000584213925096298\\
285	0.00051858575380933\\
290	0.000459632732927578\\
295	0.000405492701368321\\
300	0.000359471819535566\\
};
\addplot [color=mycolor2,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.853190928744137\\
5	0.716308099953494\\
10	0.597790301003847\\
15	0.507433257769931\\
20	0.436781526544717\\
25	0.377619913662357\\
30	0.331227247296286\\
35	0.289573318952328\\
40	0.254930400441495\\
45	0.223876868960043\\
50	0.197100154590573\\
55	0.172573059598581\\
60	0.15187951199726\\
65	0.132818286748063\\
70	0.116412818684756\\
75	0.102366658649554\\
80	0.0895517573169178\\
85	0.0782690845801202\\
90	0.0687702235364466\\
95	0.0605453637667267\\
100	0.0527692056653537\\
105	0.046279677995864\\
110	0.0409295854643531\\
115	0.0357909446748747\\
120	0.0314288015945496\\
125	0.0274914123342111\\
130	0.0242963003649855\\
135	0.0213793640114263\\
140	0.0187581964692928\\
145	0.0164488041888201\\
150	0.0145770238084191\\
155	0.0128163561542936\\
160	0.0112420570682226\\
165	0.00987137174645949\\
170	0.0087322914206499\\
175	0.0077156145719061\\
180	0.00680957150721143\\
185	0.00597542840267847\\
190	0.00526710025720474\\
195	0.00466272938916055\\
200	0.0041348624295619\\
205	0.00363724918612139\\
210	0.00320023553664209\\
215	0.00283334048484947\\
220	0.00250491767670918\\
225	0.00222873774371812\\
230	0.00195993063034286\\
235	0.00173129046297071\\
240	0.00152853335493559\\
245	0.00135295399395574\\
250	0.00120680999540491\\
255	0.00106861989226984\\
260	0.000944028799286053\\
265	0.000833414600302724\\
270	0.000735724144630847\\
275	0.000657442561550606\\
280	0.000583914431488172\\
285	0.000518384810499988\\
290	0.000459415205900953\\
295	0.000405219517447509\\
300	0.000359296128586188\\
};
\addlegendentry{$K=400$};

\addplot [color=mycolor3,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.855390165863488\\
5	0.717199588547043\\
10	0.598679521211843\\
15	0.50666073636277\\
20	0.436056587045811\\
25	0.376633528421096\\
30	0.330280264138916\\
35	0.288655011001349\\
40	0.254081635947297\\
45	0.22300664646813\\
50	0.196323134346074\\
55	0.171795623706155\\
60	0.151235903424568\\
65	0.132212617962198\\
70	0.115966050729205\\
75	0.101961984715256\\
80	0.0892145267404253\\
85	0.0781897402069122\\
90	0.068527081110355\\
95	0.0603189897359619\\
100	0.052578795466206\\
105	0.0461096327669127\\
110	0.0407746413419752\\
115	0.0356614578136092\\
120	0.0312991050085873\\
125	0.027391243542442\\
130	0.0242066269363145\\
135	0.0212956457474627\\
140	0.0186868811838104\\
145	0.0163862328644078\\
150	0.0145205626001374\\
155	0.0127684857048148\\
160	0.0111990240011519\\
165	0.00983568691987968\\
170	0.00869983626636708\\
175	0.00768637914006704\\
180	0.00678205024523127\\
185	0.00595395524043717\\
190	0.00524692559800663\\
195	0.00464344393384472\\
200	0.00411931638237435\\
205	0.00362347473821819\\
210	0.00318775018693328\\
215	0.00282092226979456\\
220	0.00249483615829437\\
225	0.0022199817964207\\
230	0.00195211138964177\\
235	0.00172467917525161\\
240	0.00152257425776662\\
245	0.00134757839571393\\
250	0.00120203870432814\\
255	0.00106497627460763\\
260	0.000940358864508797\\
265	0.000830115177177805\\
270	0.000732839377355239\\
275	0.000654860354131136\\
280	0.000581622329876766\\
285	0.000516335074475338\\
290	0.000457568271171931\\
295	0.000403665051002729\\
300	0.000357848054051724\\
};
\addplot [color=mycolor3,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.852967014323743\\
5	0.715486817998\\
10	0.597651870152298\\
15	0.507299523011594\\
20	0.436620107490143\\
25	0.377461147014222\\
30	0.331043132071505\\
35	0.289434081321329\\
40	0.254871993464684\\
45	0.223756190557617\\
50	0.19698870667604\\
55	0.172461952721709\\
60	0.151801367646401\\
65	0.132748790923661\\
70	0.116360734021818\\
75	0.102323583038331\\
80	0.0895099173785225\\
85	0.0784585027368018\\
90	0.06873975691885\\
95	0.0605198903059686\\
100	0.052748443251944\\
105	0.046260377939006\\
110	0.0409134543139719\\
115	0.0357772425130396\\
120	0.0314067774808614\\
125	0.0274803632065586\\
130	0.0242870170170513\\
135	0.0213705768293913\\
140	0.0187504961693572\\
145	0.0164426811633601\\
150	0.014568966724869\\
155	0.0128115172720475\\
160	0.0112376334037552\\
165	0.00986740827984821\\
170	0.00872887826687372\\
175	0.00771251797018794\\
180	0.00680682258869271\\
185	0.00597309882197711\\
190	0.00526512086332543\\
195	0.00465957108811473\\
200	0.0041332892229492\\
205	0.00363586737136637\\
210	0.00319894264186248\\
215	0.00283139761642345\\
220	0.00250352552567196\\
225	0.00222782629450242\\
230	0.00195916590190866\\
235	0.00173060810375251\\
240	0.00152794309061646\\
245	0.00135241092146069\\
250	0.00120633795529133\\
255	0.0010687673066535\\
260	0.000943662426255197\\
265	0.000833086760779636\\
270	0.000735432995530123\\
275	0.000657211357994324\\
280	0.000583695658805995\\
285	0.000518180651326992\\
290	0.000459241287165389\\
295	0.000405060633136984\\
300	0.000359155091024974\\
};
\addlegendentry{$K=1000$};

\end{axis}
\end{tikzpicture}%

==> 19-10-08 Final version/graphs/tikz2pdf/eigenvalues/eigenvaluesOfSigma.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0,0,0}%0.00000,0.44700,0.74100
%
\begin{tikzpicture}

\begin{axis}[%
width=\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
xmin=0,
xmax=300,
xlabel={eigenvalue index},
ymode=log,
ymin=1e-06,
ymax=1000,
yminorticks=true,
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=mycolor1,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	209.336135582511\\
2	187.536850637829\\
3	183.73196451662\\
4	165.933909412251\\
5	150.66058215411\\
6	147.742473063621\\
7	135.369127888349\\
8	131.16897584198\\
9	109.350139409312\\
10	108.47887997943\\
11	106.873853603143\\
12	99.1449355278022\\
13	95.7566408158735\\
14	77.8076550082425\\
15	77.1279442948726\\
16	73.1568163596769\\
17	72.1429141661389\\
18	65.7221277750891\\
19	64.7936072849495\\
20	56.4453977962422\\
21	53.4316781766514\\
22	51.0362765945611\\
23	46.5757646963932\\
24	44.9170595816108\\
25	41.232528651508\\
26	40.1944644116395\\
27	37.9974556451037\\
28	37.593050431783\\
29	33.1120834806314\\
30	32.1593860824133\\
31	26.6625542393675\\
32	25.8973614036002\\
33	25.3861762579731\\
34	23.9804528386554\\
35	23.5730215293401\\
36	23.359990277853\\
37	22.6532490876457\\
38	18.738870229171\\
39	18.4500372924803\\
40	16.1441818370672\\
41	15.872220715107\\
42	14.1559439001004\\
43	13.9802813189052\\
44	13.4791355818723\\
45	13.4115110164971\\
46	12.5517968205499\\
47	12.2687843181775\\
48	10.1033244479694\\
49	9.95510914045601\\
50	9.86868209277192\\
51	9.27894600749014\\
52	9.1994458827563\\
53	7.2959213799134\\
54	7.26201601082095\\
55	6.88525540598925\\
56	6.81278174267704\\
57	6.23109868337014\\
58	6.10144640550998\\
59	5.80615591209722\\
60	5.70182252172332\\
61	4.97748724774309\\
62	4.88846800336479\\
63	4.85920895215744\\
64	4.83894222597645\\
65	3.67347161619074\\
66	3.53511396887525\\
67	3.36330046419165\\
68	3.21677535024259\\
69	3.1733176991085\\
70	3.09632185689181\\
71	2.95579524408523\\
72	2.87260878254865\\
73	2.85423720381965\\
74	2.42842622254893\\
75	2.40435571560258\\
76	2.2946589435362\\
77	2.26094682624502\\
78	1.79164919146948\\
79	1.75305940311542\\
80	1.71442519641781\\
81	1.61532119784904\\
82	1.51932323098306\\
83	1.50369040011094\\
84	1.37898686658106\\
85	1.35946616785481\\
86	1.24176183417494\\
87	1.21197929863007\\
88	1.13067285739668\\
89	1.10600448793002\\
90	1.00482062585178\\
91	0.980200043679483\\
92	0.936334639350765\\
93	0.887532444601867\\
94	0.8556654848432\\
95	0.727626843628279\\
96	0.714555413934202\\
97	0.701889010444256\\
98	0.695139192694894\\
99	0.565273625208258\\
100	0.550748721355464\\
101	0.506310805659503\\
102	0.498914280142362\\
103	0.486504132909923\\
104	0.475722996125722\\
105	0.468155043694207\\
106	0.453124892016885\\
107	0.410451047852891\\
108	0.404064309183257\\
109	0.398120990182929\\
110	0.390440623033491\\
111	0.305026432481223\\
112	0.301432259915808\\
113	0.292947678911749\\
114	0.285713666725406\\
115	0.231910331207057\\
116	0.216568251820408\\
117	0.214926863185194\\
118	0.212128071023115\\
119	0.208365716049942\\
120	0.199377772982885\\
121	0.195132735602196\\
122	0.188038873828736\\
123	0.187149172327284\\
124	0.17511493622528\\
125	0.173106234689031\\
126	0.153242743763993\\
127	0.149567483801864\\
128	0.124665212600415\\
129	0.118841802456597\\
130	0.112667287055506\\
131	0.110761997515029\\
132	0.107111170736204\\
133	0.105944982261581\\
134	0.0925794431929028\\
135	0.0915669061424099\\
136	0.0769786404900289\\
137	0.075842689748883\\
138	0.0754523758887881\\
139	0.0750966022235598\\
140	0.0708810292539581\\
141	0.0701960840458445\\
142	0.0677686860950608\\
143	0.0667088054712596\\
144	0.0549527999310265\\
145	0.0535192123026823\\
146	0.0496440675855273\\
147	0.0471872358716845\\
148	0.0464561808345398\\
149	0.0457521772433598\\
150	0.045143485892636\\
151	0.0401436585932865\\
152	0.0393097870269505\\
153	0.0374287378254898\\
154	0.0369673367954435\\
155	0.0275004014622059\\
156	0.027192224190628\\
157	0.0266645982058847\\
158	0.0264239240897233\\
159	0.0255252358019609\\
160	0.0250609191590504\\
161	0.0228319120143787\\
162	0.0227809264078443\\
163	0.021583611191209\\
164	0.0211975606056378\\
165	0.0187753193625012\\
166	0.0184383973325739\\
167	0.0182798042067323\\
168	0.0180705870809209\\
169	0.0166585438583107\\
170	0.0164229603885197\\
171	0.0145471946278105\\
172	0.0140839205740977\\
173	0.0134629434656765\\
174	0.0130690580004103\\
175	0.00971794565938374\\
176	0.00964636538218579\\
177	0.00923697741646372\\
178	0.00904873512889714\\
179	0.00892738146742226\\
180	0.00869354988328364\\
181	0.00842785733178351\\
182	0.00816552064802662\\
183	0.00806321855741671\\
184	0.00738566745669157\\
185	0.00730288465056841\\
186	0.00710488034446569\\
187	0.00695462671965859\\
188	0.00601239186342659\\
189	0.00575586062813604\\
190	0.00558914556238837\\
191	0.00549034794580156\\
192	0.00511193070495102\\
193	0.00502252599987185\\
194	0.00433962049956666\\
195	0.00420105598586655\\
196	0.00372756869378614\\
197	0.00369670284195804\\
198	0.00327869948370712\\
199	0.0032520919219322\\
200	0.00324744845938799\\
201	0.00319089384922139\\
202	0.00287997334592892\\
203	0.00284512933633318\\
204	0.00256280563541174\\
205	0.00249789721333553\\
206	0.00246662092993949\\
207	0.00246080091026979\\
208	0.00225750322180392\\
209	0.00217647579644532\\
210	0.00183790126745766\\
211	0.00179998924101722\\
212	0.00176523058945998\\
213	0.00175369447566301\\
214	0.00172254257464802\\
215	0.00167343362745392\\
216	0.00149739538812696\\
217	0.00142452144217857\\
218	0.00139980676435456\\
219	0.00131990772725409\\
220	0.00128708290551841\\
221	0.001173508188405\\
222	0.00115073718587185\\
223	0.00104910145753541\\
224	0.0010290411005805\\
225	0.000891782725825204\\
226	0.000874217115439955\\
227	0.00085325048795856\\
228	0.000819704589683426\\
229	0.000710304664639155\\
230	0.000706133913784295\\
231	0.000642225462945644\\
232	0.00063221690757975\\
233	0.000577538927301217\\
234	0.000570710932931117\\
235	0.000561344564775584\\
236	0.00055032655977012\\
237	0.000545919631447557\\
238	0.00054220466694074\\
239	0.00051583982186355\\
240	0.000504298532532425\\
241	0.000495562247954099\\
242	0.000487251435247588\\
243	0.000395414863588718\\
244	0.000388106180758608\\
245	0.000372932859047769\\
246	0.000369623531759809\\
247	0.000319618034843737\\
248	0.000313249102654063\\
249	0.000277685025622901\\
250	0.000268031579062816\\
251	0.000254577995158779\\
252	0.000248460175427338\\
253	0.000219345453819093\\
254	0.000209301730686901\\
255	0.000199492334724594\\
256	0.00019570643606998\\
257	0.000192694703145467\\
258	0.000176796740956054\\
259	0.000174846281099392\\
260	0.000171106589206261\\
261	0.000169305914248727\\
262	0.000165440920726494\\
263	0.00016421354030365\\
264	0.00015794685524074\\
265	0.00015584079446901\\
266	0.000139855234497072\\
267	0.000136836169664652\\
268	0.000126827323207952\\
269	0.000123410231042152\\
270	0.000104956254374767\\
271	0.000101470593854934\\
272	9.16233557211547e-05\\
273	9.0645493464571e-05\\
274	8.32245439403213e-05\\
275	8.1973629424507e-05\\
276	7.82485233503991e-05\\
277	7.63842313195545e-05\\
278	6.998338753732e-05\\
279	6.86988503342107e-05\\
280	6.8377250514539e-05\\
281	6.66668192508118e-05\\
282	5.47780922711372e-05\\
283	5.42998025576844e-05\\
284	5.09969498802109e-05\\
285	5.08109326961006e-05\\
286	4.86273908327219e-05\\
287	4.73508654277609e-05\\
288	4.5767113039306e-05\\
289	4.56266163596427e-05\\
290	4.33495101903411e-05\\
291	4.23633658753243e-05\\
292	3.8947003383029e-05\\
293	3.74080642962811e-05\\
294	3.65572759143167e-05\\
295	3.59635224239782e-05\\
296	2.77567464698797e-05\\
297	2.74439423057806e-05\\
298	2.68564123105295e-05\\
299	2.60358224253432e-05\\
300	2.58118869306748e-05\\
};
\addlegendentry{Spectrum of $\Sigma$};

\end{axis}
\end{tikzpicture}%

==> 19-10-08 Final version/graphs/tikz2pdf/error/error_H1.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
xmin=1,
xmax=300,
xlabel={rank $r$ of the projector},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
% ylabel={error},
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black,legend pos=south west}
]
\addplot [color=red,solid,line width=1.3pt]
  table[row sep=crcr]{%
2	0.807472558348582\\
10	0.597450095193871\\
20	0.436449600392578\\
40	0.254632571595873\\
70	0.116308065139542\\
100	0.0527266117073147\\
150	0.0145619853232503\\
225	0.00222687294678219\\
300	0.000358996432617659\\
};
\addlegendentry{bound(optimal)};

\addplot [color=mycolor1,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	1.16760153905007\\
10	0.82238364014784\\
20	0.651592880219405\\
40	0.349042972853041\\
70	0.159784302146144\\
100	0.072785367877112\\
150	0.0210377229508625\\
225	0.00310296476216082\\
300	0.000496824236436204\\
};
\addlegendentry{true error, $M=1$};

\addplot [color=mycolor2,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.778206633806716\\
10	0.593908625658266\\
20	0.464003103645571\\
40	0.277980162919765\\
70	0.129204020806252\\
100	0.0617210574890085\\
150	0.0160308559360177\\
225	0.00245869355106088\\
300	0.000399047822356083\\
};
\addlegendentry{true error, $M=5$};

\addplot [color=mycolor3,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.750053098827797\\
10	0.5609924618877\\
20	0.418482493588299\\
40	0.251918994496027\\
70	0.118501963515352\\
100	0.0538698737363432\\
150	0.0148903061619574\\
225	0.00228137511073989\\
300	0.000363166986649075\\
};
\addlegendentry{true error, $M=20$};

\addplot [color=black,dashdotted,line width=2.0pt]
  table[row sep=crcr]{%
2	0.85630534968229\\
10	0.694085547674856\\
20	0.52703052321441\\
40	0.303743096880065\\
70	0.137163495684379\\
100	0.0616827327748511\\
150	0.0169459572900904\\
225	0.00257281127335595\\
300	0.000423901007739994\\
};
\addlegendentry{bound(\textit{a priori})};

\end{axis}
\end{tikzpicture}%

==> 19-10-08 Final version/graphs/tikz2pdf/error/error_H1_subD.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
xmin=1,
xmax=300,
xlabel={rank $r$ of the projector},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
% ylabel={error},
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=red,solid,line width=1.3pt]
  table[row sep=crcr]{%
2	0.217663100625997\\
10	0.0954642405127776\\
20	0.0491082382330095\\
40	0.0184546273307816\\
70	0.00480996021802693\\
100	0.00144027675331727\\
150	0.000207706756824621\\
225	1.39080076946731e-05\\
300	1.18792405053916e-06\\
};
\addlegendentry{bound(optimal)};

\addplot [color=mycolor1,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.379254144976244\\
10	0.134189765762681\\
20	0.0613031992624068\\
40	0.0272510725957513\\
70	0.00794565635790103\\
100	0.00191004501203607\\
150	0.000341152237387816\\
225	2.11569605721956e-05\\
300	1.61051760747752e-06\\
};
\addlegendentry{true error, $M=1$};

\addplot [color=mycolor2,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.207262684391605\\
10	0.0956179406656673\\
20	0.048573986821667\\
40	0.0200805941489318\\
70	0.00523940229018686\\
100	0.00165530710807594\\
150	0.00022477383976852\\
225	1.62636000453355e-05\\
300	1.42712522428855e-06\\
};
\addlegendentry{true error, $M=5$};

\addplot [color=mycolor3,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.204111293543686\\
10	0.0899831373583708\\
20	0.0469710010581219\\
40	0.0181981625543701\\
70	0.00476397369415748\\
100	0.00146680009166975\\
150	0.000206207890987376\\
225	1.49042992006038e-05\\
300	1.28456720392211e-06\\
};
\addlegendentry{true error, $M=20$};

\addplot [color=black,dashdotted,line width=2.0pt]
  table[row sep=crcr]{%
2	0.299684180173643\\
10	0.223696688248648\\
20	0.167046044342662\\
40	0.0911132718541728\\
70	0.0382884272548094\\
100	0.0172496854589005\\
150	0.00474038949244567\\
225	0.000718875553379073\\
300	0.000117896400744764\\
};
\addlegendentry{bound(\textit{a priori})};

\legend{}

\end{axis}
\end{tikzpicture}%

==> 19-10-08 Final version/graphs/tikz2pdf/error/error_Points1.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
xmin=1,
xmax=300,
xlabel={rank $r$ of the projector},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
% ylabel={error},
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=red,solid,line width=1.3pt]
  table[row sep=crcr]{%
2	0.0536736287496986\\
10	0.0295041756555123\\
20	0.0162074811796204\\
40	0.00583978133594533\\
70	0.00147408106120073\\
100	0.000395068501006725\\
150	5.14802787333588e-05\\
225	3.12185812968833e-06\\
300	2.68260147207945e-07\\
};
\addlegendentry{bound(optimal)};

\addplot [color=mycolor1,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.0631703217365317\\
10	0.0603265683689031\\
20	0.0187787276097434\\
40	0.00742084062472918\\
70	0.00197545094654398\\
100	0.000537348627082002\\
150	8.4387039741809e-05\\
225	4.54268969908211e-06\\
300	3.74075084237798e-07\\
};
\addlegendentry{true error, $M=1$};

\addplot [color=mycolor2,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.0391178994422325\\
10	0.0251589681572105\\
20	0.0156107743628942\\
40	0.00607375590189097\\
70	0.00154482123621853\\
100	0.000449879502112509\\
150	5.39442081916229e-05\\
225	3.57434448632737e-06\\
300	3.06415513039517e-07\\
};
\addlegendentry{true error, $M=5$};

\addplot [color=mycolor3,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.0386745363074597\\
10	0.0246709040425475\\
20	0.0142446123689543\\
40	0.00502674928076782\\
70	0.00144492068528846\\
100	0.000407567199277858\\
150	5.11779226245368e-05\\
225	3.31194227497593e-06\\
300	2.85000172788178e-07\\
};
\addlegendentry{true error, $M=20$};

\addplot [color=black,dashdotted,line width=2.0pt]
  table[row sep=crcr]{%
2	0.129347622262092\\
10	0.0828058265262463\\
20	0.0428187457549505\\
40	0.0208942096770329\\
70	0.0070877167566837\\
100	0.00295154753377254\\
150	0.000547404433760171\\
225	6.73650881062218e-05\\
300	1.07111254646618e-05\\
};
\addlegendentry{bound(\textit{a priori})};

\legend{}
\end{axis}
\end{tikzpicture}%

==> graphs/tikz2pdf/UB_H1/UB_H1.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.50000,0.37241}%
\definecolor{mycolor2}{rgb}{1.00000,0.10345,0.72414}%
\definecolor{mycolor3}{rgb}{1.00000,0.82759,0.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
xmin=0,
xmax=300,
xlabel={rank $r$ of the projector},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
% ylabel={upper bound},
axis background/.style={fill=white},
legend style={at={(0.03,0.03)},anchor=south west,legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=blue,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.842657915792269\\
5	0.69076411328902\\
10	0.567914384342777\\
15	0.476785924557505\\
20	0.406368006623714\\
25	0.347900785572591\\
30	0.301806303577856\\
35	0.262880488099575\\
40	0.230194014045033\\
45	0.202513741162513\\
50	0.178147717427282\\
55	0.156988342568957\\
60	0.138168781608234\\
65	0.12109181853017\\
70	0.106528926425554\\
75	0.0936889419612097\\
80	0.0822665056715205\\
85	0.0720300412809685\\
90	0.0633792683428896\\
95	0.0556873697940693\\
100	0.0485950023901831\\
105	0.0425971191201518\\
110	0.0375603788270293\\
115	0.032882828670963\\
120	0.0288230523719433\\
125	0.0252807518472025\\
130	0.0222848255191372\\
135	0.0195927755434287\\
140	0.0171930027056383\\
145	0.0150596473004764\\
150	0.0133468049840736\\
155	0.0117440098319116\\
160	0.0102925419682097\\
165	0.00903941276797616\\
170	0.0079972170917804\\
175	0.00705828060525645\\
180	0.0062173490309346\\
185	0.00546201166393073\\
190	0.00481435025622517\\
195	0.00425947959862928\\
200	0.00377806913410259\\
205	0.00332623911584736\\
210	0.00291985567274236\\
215	0.00257926568453537\\
220	0.00229218502648345\\
225	0.0020334824664312\\
230	0.00178818117580089\\
235	0.00157822061963942\\
240	0.0013953296768144\\
245	0.00123593761551859\\
250	0.00109996239613032\\
255	0.000972228122646838\\
260	0.000861333853902723\\
265	0.000759495833718544\\
270	0.000670261084633744\\
275	0.000598986120236976\\
280	0.000533115877666115\\
285	0.00047226132625629\\
290	0.000417678169458706\\
295	0.000368127814979725\\
300	0.000327672127950067\\
};
\addplot [color=blue,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.858233313722005\\
5	0.726710500676723\\
10	0.611331861835439\\
15	0.521440641551332\\
20	0.45073280005378\\
25	0.39162090729242\\
30	0.345153103193509\\
35	0.304971882449891\\
40	0.272201950431809\\
45	0.241931592771057\\
50	0.214671750368154\\
55	0.189403386423354\\
60	0.166342834561152\\
65	0.145484504191848\\
70	0.12785939489447\\
75	0.112970220789883\\
80	0.0978550357623193\\
85	0.0844639651063895\\
90	0.0741034927655092\\
95	0.0650777186878532\\
100	0.0565137933249781\\
105	0.0493996600070602\\
110	0.0436946809081395\\
115	0.0383440374648774\\
120	0.0335924620857466\\
125	0.0293265542662369\\
130	0.0259297270809694\\
135	0.0228495885241513\\
140	0.0200756147120758\\
145	0.0175363988923956\\
150	0.0155783076410874\\
155	0.0137173356801225\\
160	0.0119984449607093\\
165	0.0105420182906345\\
170	0.00933558145968237\\
175	0.00825588050195221\\
180	0.00727847411198366\\
185	0.00638489820907557\\
190	0.00563014126307845\\
195	0.00498405141256306\\
200	0.0044220138444447\\
205	0.003885310132755\\
210	0.00341673926740516\\
215	0.00302753501577763\\
220	0.00267909295708271\\
225	0.00238438762263271\\
230	0.00209486167654273\\
235	0.00185560976402689\\
240	0.00163960564885917\\
245	0.00144483951843683\\
250	0.00129168246407706\\
255	0.00114373890309044\\
260	0.00101126630068726\\
265	0.000892086551254905\\
270	0.000786292266029136\\
275	0.000704618029058656\\
280	0.000627226236147052\\
285	0.000555613875120688\\
290	0.000492746802403779\\
295	0.000434113607784357\\
300	0.000384968262383339\\
};
\addlegendentry{$K=5$};

\addplot [color=red,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.850512170978715\\
5	0.704704822813094\\
10	0.587794749289308\\
15	0.49533856183076\\
20	0.425080438191743\\
25	0.367428614993631\\
30	0.321040212251133\\
35	0.281075088566629\\
40	0.24684652965523\\
45	0.216763713443671\\
50	0.190413969097751\\
55	0.167226072559285\\
60	0.146722954921339\\
65	0.128456906202566\\
70	0.113053658425114\\
75	0.0996568602030031\\
80	0.0877291179281566\\
85	0.0766816025439446\\
90	0.0677003852937802\\
95	0.0596256659091653\\
100	0.0521824430581325\\
105	0.0457688589507645\\
110	0.0403541725575453\\
115	0.0354679665731202\\
120	0.0311037695542205\\
125	0.027215061905272\\
130	0.0240867563111981\\
135	0.0211795488558973\\
140	0.018541865662408\\
145	0.0162898122777316\\
150	0.0144080240555982\\
155	0.0126994749885521\\
160	0.0111586684930419\\
165	0.00979112418483664\\
170	0.00864364937975739\\
175	0.00765472694217975\\
180	0.00674730400455183\\
185	0.00593119823132425\\
190	0.00522002436231317\\
195	0.00461391729949155\\
200	0.00410160400566164\\
205	0.00361555638665624\\
210	0.00317669498007517\\
215	0.00280674084918528\\
220	0.00248359065132361\\
225	0.00221021578136214\\
230	0.0019487177815258\\
235	0.00171980085126473\\
240	0.00151640268202168\\
245	0.00134092390779691\\
250	0.00119793275704856\\
255	0.00106072078559652\\
260	0.000937748840516486\\
265	0.000827887326621959\\
270	0.000730628168773174\\
275	0.000651960850147478\\
280	0.000579634324411948\\
285	0.000514703528525368\\
290	0.000456163726664842\\
295	0.000402546054791443\\
300	0.000356461480351224\\
};
\addplot [color=red,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.855343515422925\\
5	0.724869593429108\\
10	0.612727575236856\\
15	0.520714012013864\\
20	0.452827595542844\\
25	0.393875659404952\\
30	0.347562169266582\\
35	0.30493893684953\\
40	0.270475138419713\\
45	0.237625916154073\\
50	0.210881081294697\\
55	0.184505415143302\\
60	0.162734053981169\\
65	0.143153568131332\\
70	0.126287500652215\\
75	0.110828825626618\\
80	0.0961926060829579\\
85	0.0837952022864943\\
90	0.0731685820971639\\
95	0.0643951565381324\\
100	0.0555736939276209\\
105	0.0486714637201366\\
110	0.0430127235608683\\
115	0.037580467399705\\
120	0.0329725867095308\\
125	0.0288496066814833\\
130	0.0256019535187486\\
135	0.0224290629797684\\
140	0.0197194190411469\\
145	0.0172799362673527\\
150	0.0153142443176654\\
155	0.0134745158263707\\
160	0.011814359465228\\
165	0.0103577623227093\\
170	0.00917769743068845\\
175	0.00809918537100417\\
180	0.0071530267468867\\
185	0.00627867478167502\\
190	0.00553283416842909\\
195	0.00488868835961701\\
200	0.00434880196089137\\
205	0.00381400169911119\\
210	0.0033564690443103\\
215	0.0029733832890057\\
220	0.0026274429146738\\
225	0.00234488091893221\\
230	0.00205828120847078\\
235	0.00181791315163297\\
240	0.00160556627062258\\
245	0.00142044980028128\\
250	0.00126984671421342\\
255	0.00112296188896457\\
260	0.000993302940352323\\
265	0.000875923354297582\\
270	0.000772835927783662\\
275	0.000690952694755479\\
280	0.000613931429928853\\
285	0.000544293067220917\\
290	0.000483015988450625\\
295	0.000426092175290265\\
300	0.000377510484782385\\
};
\addlegendentry{$K=10$};

\addplot [color=green,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.854197254907859\\
5	0.717015641320805\\
10	0.59634035068928\\
15	0.499413294138865\\
20	0.428333424520721\\
25	0.368839914040255\\
30	0.322536330839426\\
35	0.282091417730032\\
40	0.248324404494851\\
45	0.218369444101101\\
50	0.192034499612396\\
55	0.168156504880067\\
60	0.148037242228472\\
65	0.129462941372921\\
70	0.113726764304868\\
75	0.100006740570129\\
80	0.0876291445270227\\
85	0.0765842557687437\\
90	0.0673473721892849\\
95	0.0593034310290491\\
100	0.0516967704807667\\
105	0.0453185105351316\\
110	0.0400448307415058\\
115	0.0350192675684505\\
120	0.0307308448208458\\
125	0.0269164001636126\\
130	0.0237718111375801\\
135	0.0209047761567915\\
140	0.0183482271438447\\
145	0.0160932478320694\\
150	0.0142603228587902\\
155	0.0125462261165772\\
160	0.0109947189496498\\
165	0.00966226175691337\\
170	0.00854428421407931\\
175	0.00754614105559317\\
180	0.00665564156517151\\
185	0.00584764429501224\\
190	0.00515199682148927\\
195	0.00455976761707171\\
200	0.00404681372373042\\
205	0.00355901960551115\\
210	0.00312853188747008\\
215	0.00276720023033176\\
220	0.00244967361798865\\
225	0.00217965824027847\\
230	0.00191559258221392\\
235	0.00169307677352023\\
240	0.00149492354418456\\
245	0.00132340605749643\\
250	0.00117941719108671\\
255	0.00104521160923427\\
260	0.000923088794761547\\
265	0.000814938953051759\\
270	0.000719386959364935\\
275	0.00064309926084529\\
280	0.000570990551559929\\
285	0.000506878846877783\\
290	0.000449045741468337\\
295	0.000396349116198688\\
300	0.000351318234312536\\
};
\addplot [color=green,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.854271536293235\\
5	0.720938822257353\\
10	0.603114708679451\\
15	0.511065854152822\\
20	0.440297997506645\\
25	0.381167287913049\\
30	0.334852375628686\\
35	0.293337949022501\\
40	0.258378170647058\\
45	0.22683589438385\\
50	0.199507249854882\\
55	0.174596372398823\\
60	0.153595451700334\\
65	0.134275202894173\\
70	0.117690279893938\\
75	0.103466873953241\\
80	0.0904746480054325\\
85	0.0790348430749354\\
90	0.0694357121828301\\
95	0.0611490402694152\\
100	0.0532421550548823\\
105	0.0467003479778135\\
110	0.0413131134014289\\
115	0.0361059575561718\\
120	0.0317100760554909\\
125	0.0277403064309615\\
130	0.0245233024654611\\
135	0.021572687038846\\
140	0.0189333225734948\\
145	0.01660108943279\\
150	0.0147116010715365\\
155	0.012936638101999\\
160	0.011347406156045\\
165	0.00996386032057872\\
170	0.00881598219158893\\
175	0.0077871527292144\\
180	0.00687475828302562\\
185	0.00603073554702547\\
190	0.00531881587345212\\
195	0.00470683406858858\\
200	0.00417673395611798\\
205	0.00367128860650577\\
210	0.00323082673664848\\
215	0.0028601382384628\\
220	0.00252856351067335\\
225	0.002250481372068\\
230	0.00197872797106933\\
235	0.00174817575966883\\
240	0.00154384870534236\\
245	0.00136626119304521\\
250	0.00121864679197393\\
255	0.00107943756435262\\
260	0.000953263631194261\\
265	0.000841566696402781\\
270	0.000743011725841534\\
275	0.000664354421336633\\
280	0.000589681229598217\\
285	0.000523486320278789\\
290	0.000464155885235831\\
295	0.000409346047839079\\
300	0.000362893456377389\\
};
\addlegendentry{$K=30$};

\addplot [color=mycolor1,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.854386196670471\\
5	0.715829649100455\\
10	0.596337164657909\\
15	0.505257296674348\\
20	0.434551537931627\\
25	0.375840497912689\\
30	0.329091227885687\\
35	0.287796761546291\\
40	0.253487154858986\\
45	0.222831622487031\\
50	0.19593373286107\\
55	0.171856239326413\\
60	0.151301077799753\\
65	0.132345716144113\\
70	0.116050989846006\\
75	0.101997903241386\\
80	0.0893180134554772\\
85	0.0780681361709636\\
90	0.0685953782731605\\
95	0.0603877384398105\\
100	0.052672577820526\\
105	0.046161729499692\\
110	0.0408323272764152\\
115	0.0357300118287717\\
120	0.0313569850168351\\
125	0.0274416367499373\\
130	0.0242522639049808\\
135	0.0213346361314315\\
140	0.0187225610812257\\
145	0.0164133581161134\\
150	0.0145474214816311\\
155	0.01279441495011\\
160	0.0112216350886429\\
165	0.0098576077552613\\
170	0.00871647853622832\\
175	0.0077007169598588\\
180	0.00679606340443839\\
185	0.00596871467957036\\
190	0.00525736485084279\\
195	0.00465118921648993\\
200	0.00412990929599793\\
205	0.00363186289061616\\
210	0.00319393569100844\\
215	0.00282538487588462\\
220	0.00249968941170571\\
225	0.00222490526771252\\
230	0.00195610944278869\\
235	0.0017284179297172\\
240	0.00152598562470489\\
245	0.00135011845307759\\
250	0.00120416834912026\\
255	0.00106666276507667\\
260	0.000942489957259844\\
265	0.000831974240424698\\
270	0.000734432222869185\\
275	0.000656132863661093\\
280	0.000582842687974233\\
285	0.000517338293399388\\
290	0.000458485540542471\\
295	0.000404681489306519\\
300	0.000358525052979575\\
};
\addplot [color=mycolor1,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.853612718684342\\
5	0.716122542775951\\
10	0.598343490726109\\
15	0.508100273854599\\
20	0.437429247185325\\
25	0.37831299337161\\
30	0.331995639706559\\
35	0.290444719574667\\
40	0.2558102468566\\
45	0.224630544411742\\
50	0.197707075621589\\
55	0.173045583837339\\
60	0.152329444559517\\
65	0.133120852214766\\
70	0.116674629645553\\
75	0.102613486486817\\
80	0.0897623029108835\\
85	0.0784644201747734\\
90	0.0689223517786045\\
95	0.0606960007209518\\
100	0.0528856073931253\\
105	0.0463870020985316\\
110	0.0410315119051452\\
115	0.0358655495010453\\
120	0.0314980584533803\\
125	0.0275468955104903\\
130	0.0243485092274989\\
135	0.0214278854158599\\
140	0.018796810386387\\
145	0.0164774154883472\\
150	0.0146033015674753\\
155	0.0128439669622764\\
160	0.0112651898774632\\
165	0.00989038705871587\\
170	0.00874914359348096\\
175	0.00773155219608285\\
180	0.00682376333010509\\
185	0.00598693047467329\\
190	0.00527766953456218\\
195	0.00467177462688175\\
200	0.0041437950750276\\
205	0.00364445619186028\\
210	0.00320665092965731\\
215	0.00283843431808208\\
220	0.00250948313530694\\
225	0.002233491085547\\
230	0.00196402968397093\\
235	0.00173481246953296\\
240	0.00153159338331823\\
245	0.00135573646169466\\
250	0.00120928658783182\\
255	0.00107080798966196\\
260	0.000945943900016803\\
265	0.000835083336648327\\
270	0.000737240704930835\\
275	0.000658961819804986\\
280	0.000585130204741495\\
285	0.00051943765284706\\
290	0.000460388465159522\\
295	0.000406074898741922\\
300	0.000360054511064979\\
};
\addlegendentry{$K=100$};

\addplot [color=mycolor2,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.854439098991967\\
5	0.717314039650185\\
10	0.598999906232932\\
15	0.507625162631154\\
20	0.437175784457431\\
25	0.377904176170278\\
30	0.331311201205422\\
35	0.289702904573772\\
40	0.254872064554143\\
45	0.223864678259842\\
50	0.196988836467743\\
55	0.172622774019459\\
60	0.151929224683754\\
65	0.132865093949645\\
70	0.116447433279757\\
75	0.10240101224587\\
80	0.0895604541466094\\
85	0.0782618616135494\\
90	0.0687776858075612\\
95	0.0605399467241175\\
100	0.0528011075011571\\
105	0.0462856095603078\\
110	0.0409424038120007\\
115	0.0358083132010283\\
120	0.0314381319041955\\
125	0.027509517282882\\
130	0.0243103362246009\\
135	0.0213852088507478\\
140	0.018766798421279\\
145	0.0164536087038316\\
150	0.0145890214124435\\
155	0.0128245668503279\\
160	0.0112457331747136\\
165	0.00987848361364716\\
170	0.00873970525857594\\
175	0.00771810401514336\\
180	0.00681152970316948\\
185	0.00598098247437613\\
190	0.00526993326255038\\
195	0.00466607400740655\\
200	0.00413798758146018\\
205	0.00364002499811922\\
210	0.00320119482997444\\
215	0.0028345259470569\\
220	0.0025065699033971\\
225	0.00223012883874875\\
230	0.00196059980242888\\
235	0.00173235763439631\\
240	0.00152952119928271\\
245	0.00135371910019878\\
250	0.00120746291525698\\
255	0.00106932620178584\\
260	0.000944559887812081\\
265	0.000833837423747803\\
270	0.000736177656942217\\
275	0.000657895529395546\\
280	0.000584213925096298\\
285	0.00051858575380933\\
290	0.000459632732927578\\
295	0.000405492701368321\\
300	0.000359471819535566\\
};
\addplot [color=mycolor2,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.853190928744137\\
5	0.716308099953494\\
10	0.597790301003847\\
15	0.507433257769931\\
20	0.436781526544717\\
25	0.377619913662357\\
30	0.331227247296286\\
35	0.289573318952328\\
40	0.254930400441495\\
45	0.223876868960043\\
50	0.197100154590573\\
55	0.172573059598581\\
60	0.15187951199726\\
65	0.132818286748063\\
70	0.116412818684756\\
75	0.102366658649554\\
80	0.0895517573169178\\
85	0.0782690845801202\\
90	0.0687702235364466\\
95	0.0605453637667267\\
100	0.0527692056653537\\
105	0.046279677995864\\
110	0.0409295854643531\\
115	0.0357909446748747\\
120	0.0314288015945496\\
125	0.0274914123342111\\
130	0.0242963003649855\\
135	0.0213793640114263\\
140	0.0187581964692928\\
145	0.0164488041888201\\
150	0.0145770238084191\\
155	0.0128163561542936\\
160	0.0112420570682226\\
165	0.00987137174645949\\
170	0.0087322914206499\\
175	0.0077156145719061\\
180	0.00680957150721143\\
185	0.00597542840267847\\
190	0.00526710025720474\\
195	0.00466272938916055\\
200	0.0041348624295619\\
205	0.00363724918612139\\
210	0.00320023553664209\\
215	0.00283334048484947\\
220	0.00250491767670918\\
225	0.00222873774371812\\
230	0.00195993063034286\\
235	0.00173129046297071\\
240	0.00152853335493559\\
245	0.00135295399395574\\
250	0.00120680999540491\\
255	0.00106861989226984\\
260	0.000944028799286053\\
265	0.000833414600302724\\
270	0.000735724144630847\\
275	0.000657442561550606\\
280	0.000583914431488172\\
285	0.000518384810499988\\
290	0.000459415205900953\\
295	0.000405219517447509\\
300	0.000359296128586188\\
};
\addlegendentry{$K=400$};

\addplot [color=mycolor3,dashed,line width=1.3pt,forget plot]
  table[row sep=crcr]{%
1	0.855390165863488\\
5	0.717199588547043\\
10	0.598679521211843\\
15	0.50666073636277\\
20	0.436056587045811\\
25	0.376633528421096\\
30	0.330280264138916\\
35	0.288655011001349\\
40	0.254081635947297\\
45	0.22300664646813\\
50	0.196323134346074\\
55	0.171795623706155\\
60	0.151235903424568\\
65	0.132212617962198\\
70	0.115966050729205\\
75	0.101961984715256\\
80	0.0892145267404253\\
85	0.0781897402069122\\
90	0.068527081110355\\
95	0.0603189897359619\\
100	0.052578795466206\\
105	0.0461096327669127\\
110	0.0407746413419752\\
115	0.0356614578136092\\
120	0.0312991050085873\\
125	0.027391243542442\\
130	0.0242066269363145\\
135	0.0212956457474627\\
140	0.0186868811838104\\
145	0.0163862328644078\\
150	0.0145205626001374\\
155	0.0127684857048148\\
160	0.0111990240011519\\
165	0.00983568691987968\\
170	0.00869983626636708\\
175	0.00768637914006704\\
180	0.00678205024523127\\
185	0.00595395524043717\\
190	0.00524692559800663\\
195	0.00464344393384472\\
200	0.00411931638237435\\
205	0.00362347473821819\\
210	0.00318775018693328\\
215	0.00282092226979456\\
220	0.00249483615829437\\
225	0.0022199817964207\\
230	0.00195211138964177\\
235	0.00172467917525161\\
240	0.00152257425776662\\
245	0.00134757839571393\\
250	0.00120203870432814\\
255	0.00106497627460763\\
260	0.000940358864508797\\
265	0.000830115177177805\\
270	0.000732839377355239\\
275	0.000654860354131136\\
280	0.000581622329876766\\
285	0.000516335074475338\\
290	0.000457568271171931\\
295	0.000403665051002729\\
300	0.000357848054051724\\
};
\addplot [color=mycolor3,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	0.852967014323743\\
5	0.715486817998\\
10	0.597651870152298\\
15	0.507299523011594\\
20	0.436620107490143\\
25	0.377461147014222\\
30	0.331043132071505\\
35	0.289434081321329\\
40	0.254871993464684\\
45	0.223756190557617\\
50	0.19698870667604\\
55	0.172461952721709\\
60	0.151801367646401\\
65	0.132748790923661\\
70	0.116360734021818\\
75	0.102323583038331\\
80	0.0895099173785225\\
85	0.0784585027368018\\
90	0.06873975691885\\
95	0.0605198903059686\\
100	0.052748443251944\\
105	0.046260377939006\\
110	0.0409134543139719\\
115	0.0357772425130396\\
120	0.0314067774808614\\
125	0.0274803632065586\\
130	0.0242870170170513\\
135	0.0213705768293913\\
140	0.0187504961693572\\
145	0.0164426811633601\\
150	0.014568966724869\\
155	0.0128115172720475\\
160	0.0112376334037552\\
165	0.00986740827984821\\
170	0.00872887826687372\\
175	0.00771251797018794\\
180	0.00680682258869271\\
185	0.00597309882197711\\
190	0.00526512086332543\\
195	0.00465957108811473\\
200	0.0041332892229492\\
205	0.00363586737136637\\
210	0.00319894264186248\\
215	0.00283139761642345\\
220	0.00250352552567196\\
225	0.00222782629450242\\
230	0.00195916590190866\\
235	0.00173060810375251\\
240	0.00152794309061646\\
245	0.00135241092146069\\
250	0.00120633795529133\\
255	0.0010687673066535\\
260	0.000943662426255197\\
265	0.000833086760779636\\
270	0.000735432995530123\\
275	0.000657211357994324\\
280	0.000583695658805995\\
285	0.000518180651326992\\
290	0.000459241287165389\\
295	0.000405060633136984\\
300	0.000359155091024974\\
};
\addlegendentry{$K=1000$};

\end{axis}
\end{tikzpicture}%

==> graphs/tikz2pdf/eigenvalues/eigenvaluesOfSigma.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0,0,0}%0.00000,0.44700,0.74100
%
\begin{tikzpicture}

\begin{axis}[%
width=\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
xmin=0,
xmax=300,
xlabel={eigenvalue index},
ymode=log,
ymin=1e-06,
ymax=1000,
yminorticks=true,
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=mycolor1,solid,line width=1.3pt]
  table[row sep=crcr]{%
1	209.336135582511\\
2	187.536850637829\\
3	183.73196451662\\
4	165.933909412251\\
5	150.66058215411\\
6	147.742473063621\\
7	135.369127888349\\
8	131.16897584198\\
9	109.350139409312\\
10	108.47887997943\\
11	106.873853603143\\
12	99.1449355278022\\
13	95.7566408158735\\
14	77.8076550082425\\
15	77.1279442948726\\
16	73.1568163596769\\
17	72.1429141661389\\
18	65.7221277750891\\
19	64.7936072849495\\
20	56.4453977962422\\
21	53.4316781766514\\
22	51.0362765945611\\
23	46.5757646963932\\
24	44.9170595816108\\
25	41.232528651508\\
26	40.1944644116395\\
27	37.9974556451037\\
28	37.593050431783\\
29	33.1120834806314\\
30	32.1593860824133\\
31	26.6625542393675\\
32	25.8973614036002\\
33	25.3861762579731\\
34	23.9804528386554\\
35	23.5730215293401\\
36	23.359990277853\\
37	22.6532490876457\\
38	18.738870229171\\
39	18.4500372924803\\
40	16.1441818370672\\
41	15.872220715107\\
42	14.1559439001004\\
43	13.9802813189052\\
44	13.4791355818723\\
45	13.4115110164971\\
46	12.5517968205499\\
47	12.2687843181775\\
48	10.1033244479694\\
49	9.95510914045601\\
50	9.86868209277192\\
51	9.27894600749014\\
52	9.1994458827563\\
53	7.2959213799134\\
54	7.26201601082095\\
55	6.88525540598925\\
56	6.81278174267704\\
57	6.23109868337014\\
58	6.10144640550998\\
59	5.80615591209722\\
60	5.70182252172332\\
61	4.97748724774309\\
62	4.88846800336479\\
63	4.85920895215744\\
64	4.83894222597645\\
65	3.67347161619074\\
66	3.53511396887525\\
67	3.36330046419165\\
68	3.21677535024259\\
69	3.1733176991085\\
70	3.09632185689181\\
71	2.95579524408523\\
72	2.87260878254865\\
73	2.85423720381965\\
74	2.42842622254893\\
75	2.40435571560258\\
76	2.2946589435362\\
77	2.26094682624502\\
78	1.79164919146948\\
79	1.75305940311542\\
80	1.71442519641781\\
81	1.61532119784904\\
82	1.51932323098306\\
83	1.50369040011094\\
84	1.37898686658106\\
85	1.35946616785481\\
86	1.24176183417494\\
87	1.21197929863007\\
88	1.13067285739668\\
89	1.10600448793002\\
90	1.00482062585178\\
91	0.980200043679483\\
92	0.936334639350765\\
93	0.887532444601867\\
94	0.8556654848432\\
95	0.727626843628279\\
96	0.714555413934202\\
97	0.701889010444256\\
98	0.695139192694894\\
99	0.565273625208258\\
100	0.550748721355464\\
101	0.506310805659503\\
102	0.498914280142362\\
103	0.486504132909923\\
104	0.475722996125722\\
105	0.468155043694207\\
106	0.453124892016885\\
107	0.410451047852891\\
108	0.404064309183257\\
109	0.398120990182929\\
110	0.390440623033491\\
111	0.305026432481223\\
112	0.301432259915808\\
113	0.292947678911749\\
114	0.285713666725406\\
115	0.231910331207057\\
116	0.216568251820408\\
117	0.214926863185194\\
118	0.212128071023115\\
119	0.208365716049942\\
120	0.199377772982885\\
121	0.195132735602196\\
122	0.188038873828736\\
123	0.187149172327284\\
124	0.17511493622528\\
125	0.173106234689031\\
126	0.153242743763993\\
127	0.149567483801864\\
128	0.124665212600415\\
129	0.118841802456597\\
130	0.112667287055506\\
131	0.110761997515029\\
132	0.107111170736204\\
133	0.105944982261581\\
134	0.0925794431929028\\
135	0.0915669061424099\\
136	0.0769786404900289\\
137	0.075842689748883\\
138	0.0754523758887881\\
139	0.0750966022235598\\
140	0.0708810292539581\\
141	0.0701960840458445\\
142	0.0677686860950608\\
143	0.0667088054712596\\
144	0.0549527999310265\\
145	0.0535192123026823\\
146	0.0496440675855273\\
147	0.0471872358716845\\
148	0.0464561808345398\\
149	0.0457521772433598\\
150	0.045143485892636\\
151	0.0401436585932865\\
152	0.0393097870269505\\
153	0.0374287378254898\\
154	0.0369673367954435\\
155	0.0275004014622059\\
156	0.027192224190628\\
157	0.0266645982058847\\
158	0.0264239240897233\\
159	0.0255252358019609\\
160	0.0250609191590504\\
161	0.0228319120143787\\
162	0.0227809264078443\\
163	0.021583611191209\\
164	0.0211975606056378\\
165	0.0187753193625012\\
166	0.0184383973325739\\
167	0.0182798042067323\\
168	0.0180705870809209\\
169	0.0166585438583107\\
170	0.0164229603885197\\
171	0.0145471946278105\\
172	0.0140839205740977\\
173	0.0134629434656765\\
174	0.0130690580004103\\
175	0.00971794565938374\\
176	0.00964636538218579\\
177	0.00923697741646372\\
178	0.00904873512889714\\
179	0.00892738146742226\\
180	0.00869354988328364\\
181	0.00842785733178351\\
182	0.00816552064802662\\
183	0.00806321855741671\\
184	0.00738566745669157\\
185	0.00730288465056841\\
186	0.00710488034446569\\
187	0.00695462671965859\\
188	0.00601239186342659\\
189	0.00575586062813604\\
190	0.00558914556238837\\
191	0.00549034794580156\\
192	0.00511193070495102\\
193	0.00502252599987185\\
194	0.00433962049956666\\
195	0.00420105598586655\\
196	0.00372756869378614\\
197	0.00369670284195804\\
198	0.00327869948370712\\
199	0.0032520919219322\\
200	0.00324744845938799\\
201	0.00319089384922139\\
202	0.00287997334592892\\
203	0.00284512933633318\\
204	0.00256280563541174\\
205	0.00249789721333553\\
206	0.00246662092993949\\
207	0.00246080091026979\\
208	0.00225750322180392\\
209	0.00217647579644532\\
210	0.00183790126745766\\
211	0.00179998924101722\\
212	0.00176523058945998\\
213	0.00175369447566301\\
214	0.00172254257464802\\
215	0.00167343362745392\\
216	0.00149739538812696\\
217	0.00142452144217857\\
218	0.00139980676435456\\
219	0.00131990772725409\\
220	0.00128708290551841\\
221	0.001173508188405\\
222	0.00115073718587185\\
223	0.00104910145753541\\
224	0.0010290411005805\\
225	0.000891782725825204\\
226	0.000874217115439955\\
227	0.00085325048795856\\
228	0.000819704589683426\\
229	0.000710304664639155\\
230	0.000706133913784295\\
231	0.000642225462945644\\
232	0.00063221690757975\\
233	0.000577538927301217\\
234	0.000570710932931117\\
235	0.000561344564775584\\
236	0.00055032655977012\\
237	0.000545919631447557\\
238	0.00054220466694074\\
239	0.00051583982186355\\
240	0.000504298532532425\\
241	0.000495562247954099\\
242	0.000487251435247588\\
243	0.000395414863588718\\
244	0.000388106180758608\\
245	0.000372932859047769\\
246	0.000369623531759809\\
247	0.000319618034843737\\
248	0.000313249102654063\\
249	0.000277685025622901\\
250	0.000268031579062816\\
251	0.000254577995158779\\
252	0.000248460175427338\\
253	0.000219345453819093\\
254	0.000209301730686901\\
255	0.000199492334724594\\
256	0.00019570643606998\\
257	0.000192694703145467\\
258	0.000176796740956054\\
259	0.000174846281099392\\
260	0.000171106589206261\\
261	0.000169305914248727\\
262	0.000165440920726494\\
263	0.00016421354030365\\
264	0.00015794685524074\\
265	0.00015584079446901\\
266	0.000139855234497072\\
267	0.000136836169664652\\
268	0.000126827323207952\\
269	0.000123410231042152\\
270	0.000104956254374767\\
271	0.000101470593854934\\
272	9.16233557211547e-05\\
273	9.0645493464571e-05\\
274	8.32245439403213e-05\\
275	8.1973629424507e-05\\
276	7.82485233503991e-05\\
277	7.63842313195545e-05\\
278	6.998338753732e-05\\
279	6.86988503342107e-05\\
280	6.8377250514539e-05\\
281	6.66668192508118e-05\\
282	5.47780922711372e-05\\
283	5.42998025576844e-05\\
284	5.09969498802109e-05\\
285	5.08109326961006e-05\\
286	4.86273908327219e-05\\
287	4.73508654277609e-05\\
288	4.5767113039306e-05\\
289	4.56266163596427e-05\\
290	4.33495101903411e-05\\
291	4.23633658753243e-05\\
292	3.8947003383029e-05\\
293	3.74080642962811e-05\\
294	3.65572759143167e-05\\
295	3.59635224239782e-05\\
296	2.77567464698797e-05\\
297	2.74439423057806e-05\\
298	2.68564123105295e-05\\
299	2.60358224253432e-05\\
300	2.58118869306748e-05\\
};
\addlegendentry{Spectrum of $\Sigma$};

\end{axis}
\end{tikzpicture}%

==> graphs/tikz2pdf/error/error_H1.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
xmin=1,
xmax=300,
xlabel={rank $r$ of the projector},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
% ylabel={error},
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black,legend pos=south west}
]
\addplot [color=red,solid,line width=1.3pt]
  table[row sep=crcr]{%
2	0.807472558348582\\
10	0.597450095193871\\
20	0.436449600392578\\
40	0.254632571595873\\
70	0.116308065139542\\
100	0.0527266117073147\\
150	0.0145619853232503\\
225	0.00222687294678219\\
300	0.000358996432617659\\
};
\addlegendentry{bound(optimal)};

\addplot [color=mycolor1,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	1.16760153905007\\
10	0.82238364014784\\
20	0.651592880219405\\
40	0.349042972853041\\
70	0.159784302146144\\
100	0.072785367877112\\
150	0.0210377229508625\\
225	0.00310296476216082\\
300	0.000496824236436204\\
};
\addlegendentry{true error, $M=1$};

\addplot [color=mycolor2,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.778206633806716\\
10	0.593908625658266\\
20	0.464003103645571\\
40	0.277980162919765\\
70	0.129204020806252\\
100	0.0617210574890085\\
150	0.0160308559360177\\
225	0.00245869355106088\\
300	0.000399047822356083\\
};
\addlegendentry{true error, $M=5$};

\addplot [color=mycolor3,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.750053098827797\\
10	0.5609924618877\\
20	0.418482493588299\\
40	0.251918994496027\\
70	0.118501963515352\\
100	0.0538698737363432\\
150	0.0148903061619574\\
225	0.00228137511073989\\
300	0.000363166986649075\\
};
\addlegendentry{true error, $M=20$};

\addplot [color=black,dashdotted,line width=2.0pt]
  table[row sep=crcr]{%
2	0.85630534968229\\
10	0.694085547674856\\
20	0.52703052321441\\
40	0.303743096880065\\
70	0.137163495684379\\
100	0.0616827327748511\\
150	0.0169459572900904\\
225	0.00257281127335595\\
300	0.000423901007739994\\
};
\addlegendentry{bound(\textit{a priori})};

\end{axis}
\end{tikzpicture}%

==> graphs/tikz2pdf/error/error_H1_subD.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
xmin=1,
xmax=300,
xlabel={rank $r$ of the projector},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
% ylabel={error},
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=red,solid,line width=1.3pt]
  table[row sep=crcr]{%
2	0.217663100625997\\
10	0.0954642405127776\\
20	0.0491082382330095\\
40	0.0184546273307816\\
70	0.00480996021802693\\
100	0.00144027675331727\\
150	0.000207706756824621\\
225	1.39080076946731e-05\\
300	1.18792405053916e-06\\
};
\addlegendentry{bound(optimal)};

\addplot [color=mycolor1,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.379254144976244\\
10	0.134189765762681\\
20	0.0613031992624068\\
40	0.0272510725957513\\
70	0.00794565635790103\\
100	0.00191004501203607\\
150	0.000341152237387816\\
225	2.11569605721956e-05\\
300	1.61051760747752e-06\\
};
\addlegendentry{true error, $M=1$};

\addplot [color=mycolor2,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.207262684391605\\
10	0.0956179406656673\\
20	0.048573986821667\\
40	0.0200805941489318\\
70	0.00523940229018686\\
100	0.00165530710807594\\
150	0.00022477383976852\\
225	1.62636000453355e-05\\
300	1.42712522428855e-06\\
};
\addlegendentry{true error, $M=5$};

\addplot [color=mycolor3,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.204111293543686\\
10	0.0899831373583708\\
20	0.0469710010581219\\
40	0.0181981625543701\\
70	0.00476397369415748\\
100	0.00146680009166975\\
150	0.000206207890987376\\
225	1.49042992006038e-05\\
300	1.28456720392211e-06\\
};
\addlegendentry{true error, $M=20$};

\addplot [color=black,dashdotted,line width=2.0pt]
  table[row sep=crcr]{%
2	0.299684180173643\\
10	0.223696688248648\\
20	0.167046044342662\\
40	0.0911132718541728\\
70	0.0382884272548094\\
100	0.0172496854589005\\
150	0.00474038949244567\\
225	0.000718875553379073\\
300	0.000117896400744764\\
};
\addlegendentry{bound(\textit{a priori})};

\legend{}

\end{axis}
\end{tikzpicture}%

==> graphs/tikz2pdf/error/error_Points1.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
xmin=1,
xmax=300,
xlabel={rank $r$ of the projector},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
% ylabel={error},
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=red,solid,line width=1.3pt]
  table[row sep=crcr]{%
2	0.0536736287496986\\
10	0.0295041756555123\\
20	0.0162074811796204\\
40	0.00583978133594533\\
70	0.00147408106120073\\
100	0.000395068501006725\\
150	5.14802787333588e-05\\
225	3.12185812968833e-06\\
300	2.68260147207945e-07\\
};
\addlegendentry{bound(optimal)};

\addplot [color=mycolor1,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.0631703217365317\\
10	0.0603265683689031\\
20	0.0187787276097434\\
40	0.00742084062472918\\
70	0.00197545094654398\\
100	0.000537348627082002\\
150	8.4387039741809e-05\\
225	4.54268969908211e-06\\
300	3.74075084237798e-07\\
};
\addlegendentry{true error, $M=1$};

\addplot [color=mycolor2,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.0391178994422325\\
10	0.0251589681572105\\
20	0.0156107743628942\\
40	0.00607375590189097\\
70	0.00154482123621853\\
100	0.000449879502112509\\
150	5.39442081916229e-05\\
225	3.57434448632737e-06\\
300	3.06415513039517e-07\\
};
\addlegendentry{true error, $M=5$};

\addplot [color=mycolor3,dashed,line width=1.5pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
2	0.0386745363074597\\
10	0.0246709040425475\\
20	0.0142446123689543\\
40	0.00502674928076782\\
70	0.00144492068528846\\
100	0.000407567199277858\\
150	5.11779226245368e-05\\
225	3.31194227497593e-06\\
300	2.85000172788178e-07\\
};
\addlegendentry{true error, $M=20$};

\addplot [color=black,dashdotted,line width=2.0pt]
  table[row sep=crcr]{%
2	0.129347622262092\\
10	0.0828058265262463\\
20	0.0428187457549505\\
40	0.0208942096770329\\
70	0.0070877167566837\\
100	0.00295154753377254\\
150	0.000547404433760171\\
225	6.73650881062218e-05\\
300	1.07111254646618e-05\\
};
\addlegendentry{bound(\textit{a priori})};

\legend{}
\end{axis}
\end{tikzpicture}%
